A Unified Dual Method for Matching Problems

Matching problems are ubiquitous in data science as they enable the alignment of structured objects and distributions. While existing solvers are often tailored to specific matching formulations, we unify a broad class of such problems within a common mathematical and optimization framework based on duality theory. Theoretically, we demonstrate that matching objectives decomposable as a difference of convex (DC) functions can be recast as implicit registration problems. This connection links matching to another well-studied class of objectives and yields a dual formulation amenable to natural optimization strategies. We then apply these findings to quadratic matching (QM) problems, which admit DC decompositions and for which we provide extensive convergence guarantees. Our framework applies to Gromov-Wasserstein (GW), as well as its unbalanced formulation and several variants, which are increasingly popular QM problems. Numerically, we implement our algorithms at scale for various data modalities such as graphs, point clouds, meshes, and word embeddings. Finally, our modular approach allows us to explore new formulations such as fracture matching, broadening the scope of problems that can be addressed within this framework..

==> block_proj.tex <==
\begin{algorithm}[H]
    \caption{$\texttt{Block-Proj}$ implementation.}
    \label{alg:block_proj}
    \KwIn{$\Gamma = (\Gamma_1,\dots, \Gamma_L)$, $\Xi = (\Xi_1,\dots,\Xi_K)$, $\Phi_{A,1},\dots, \Phi_{A,K}$; $\Psi_{A,1},\dots, \Psi_{A,K}$, $\Phi_{B,1},\dots, \Phi_{B,L}$, $\Psi_{B,1},\dots, \Psi_{B,L}$.}
    \KwOut{$\Omega_1,\dots, \Omega_K$} 
    \For{$k = 0, \dots, K$}{
        $\Omega_k \gets \texttt{Sink.Corr(} \Phi_k, \Psi_k\texttt{)}$\;
    }
\end{algorithm}

==> block_separable.tex <==
Theorem~\ref{thm:qot_as_registration} states the existence of embedding functions such that $\Reg\QM$ rewrites as our new formulas.
In this section, we explicit how to obtain these embeddings from the block-decomposition of the operators $A$ and $B$.
In the following, given a sequence $x_1 \in \Hilb_1,\dots, x_n \in \Hilb_n$ of vectors in distinct Hilbert spaces, we use the following matrix notation to denote their direct sum:
\begin{equation*}
   \begin{pmatrix} x_1\\ 
     \dots \\ 
    x_n \\
    \end{pmatrix} := x_1 \oplus \dots \oplus x_n \in \Hilb_1 \oplus \dots\oplus \Hilb_n. 
\end{equation*}
Informally, this corresponds to the concatenation of the vectors $x_1, \dots, x_n$ and describes a block-structured space.
It comes with a natural scalar product:
\begin{equation*}
    \scal{   \begin{pmatrix} x_1\\ 
     \dots \\ 
    x_n \\
    \end{pmatrix},  
    \begin{pmatrix} y_1\\ 
     \dots \\ 
    y_n \\
    \end{pmatrix} } = \scal{x_1,y_1} + \dots + \scal{x_n, y_n}.
\end{equation*}
For any $\Hilb_\X = \Hilb_{\X,1} \oplus \dots \oplus \Hilb_{\X,n}$ and $\Hilb_\Y = \Hilb_{\Y,1} \oplus \dots \oplus \Hilb_{\Y,n}$,
we denote the set of \emph{block-wise} Hilbert-Schmidt operators from $\Hilb_\Y$ to $\Hilb_\X$ as:
\begin{equation*}
    \HS_{\oplus}(\Hilb_\Y, \Hilb_\X) := \HS(\Hilb_{\Y,1}, \Hilb_{\X,1}) \oplus \dots \oplus \HS(\Hilb_{\Y,n}, \Hilb_{\X,n}) \subset \HS(\Hilb_\Y, \Hilb_\X),
\end{equation*}
where any $\Gamma = \Gamma_1,\dots, \Gamma_n \in  \HS_{\oplus}(\Hilb_\Y, \Hilb_\X)$ acts on $\Hilb_\Y$ as follows:
\begin{equation*}
\Gamma \cdot
\begin{pmatrix}
    y_1 \\
    \dots \\
    y_n
\end{pmatrix} = 
\begin{pmatrix}
    \Gamma_1 y_1 \\
    \dots \\
    \Gamma_n y_n
\end{pmatrix} \in \Hilb_\X.
\end{equation*}
We now assume that $A$ and $B$ are block-separable in the sense of \cref{definition:separable}.
First, note that block-separability is equivalent to the existence of separable functions $A_i : \X \times \Y \to \Hilb_{A,i}$ and $B_j: \X \times \Y \to \Hilb_{B,j}$ such that, for all $x \in \X$ and all $y \in \Y$:
\begin{equation*}
 A(x,y) = \begin{pmatrix} A_1(x,y)\\ 
     \dots \\ 
    A_\KK(x,y) \\
    \end{pmatrix} 
    \quad \text{ and } \quad  B(x, y) = \begin{pmatrix} B_1(x,y) \\ 
     \dots \\ 
    B_\LL(x,y) \\
    \end{pmatrix}.
\end{equation*}
Since each $A_i$ and $B_j$ is separable, we can write for all $x \in \X$, $y \in \Y$ and all $1 \leq i \leq \KK$, $1 \leq j \leq \LL$:
\begin{align*}
    A_{i}(x,y) = \Phi_{A,i}(x) \Psi_{A,i}(y)^\top & &\text{ where } & &\Phi_{A,i}(x) \in \Hilb^{\Phi}_{A,i} && \text{ and } && \Psi_{A,i}(y) \in \Hilb^{\Psi}_{A,i}, \\
    B_{j}(x,y) = \Phi_{B,j}(x) \Psi_{B,j}(y)^\top && \text{ where } && \Phi_{B,j}(x) \in \Hilb^{\Phi}_{B,j} && \text{ and } && \Psi_{B,j}(y) \in \Hilb^{\Psi}_{B,j}.
\end{align*}
Therefore, for each $x \in \X$ and $y \in \Y$, we have:
\begin{equation}
\label{eq:block_separable_ops}
    A(x, y) = \begin{pmatrix} \Phi_{A,1}(x)\Psi_{A,1}(y)^{\top} \\ 
     \dots \\ 
    \Phi_{A,K}(x)\Psi_{A,K}(y)^{\top} \\
    \end{pmatrix} 
    \quad \text{ and } \quad  B(x, y) = \begin{pmatrix} \Phi_{B,1}(x)\Psi_{B,1}(y)^{\top} \\ 
     \dots \\ 
    \Phi_{B,L}(x)\Psi_{B,L}(y)^{\top} \\
    \end{pmatrix}.
\end{equation}
For all $x \in \X$ and $y \in \Y$, we also define the concatenated embeddings:
\begin{equation*}
    \Phi_A(x) = \begin{pmatrix} \Phi_{A,1}(x) \\ \dots \\ \Phi_{A,\KK}(x) \end{pmatrix}, 
    \Psi_A(y) = \begin{pmatrix} \Psi_{A,1}(y) \\ \dots \\ \Psi_{A,\KK}(y) \end{pmatrix}, 
    \Phi_{A}(x) = \begin{pmatrix} \Phi_{A,1}(x) \\ \dots \\ \Phi_{A,\KK}(x) \end{pmatrix}, 
    \Psi_B(y) = \begin{pmatrix} \Psi_{B,1}(y) \\ \dots \\ \Psi_{B,\LL}(y) \end{pmatrix}.
\end{equation*}
With these notations, \cref{thm:qot_as_registration} can be explicited as follow:

\begin{theorem}
\label{thm:qot_as_registration_blockseparable}
Let assume that $B$ is block-separable with concatenated embeddings $\Phi_{B} \in \Hilb^{\Phi}_B$ and $\Psi_{B} \in \Hilb^{\Psi}_B$.
Let $\mathbf{R}$ and $\mathbf{S}$ be as in \cref{prop:outer_gamma}.
Then, the $\Reg\QM$ problem is equivalent to:
\begin{equation*}
        \min_{\Gamma \in \HS_{\oplus}(\Hilb^{\Psi}_B, \Hilb^\Phi_B)} ~~ \min_{\pi \in \measplus{\X \times \Y}}\; - \int \scal{\Phi_B(x), \Gamma \cdot \Psi_B(y)} \diff \pi(x,y) + \mathbf{R}(\pi) + \mathbf{S}(\Gamma).
\end{equation*}
\end{theorem}

We provide the proof of this result in \cref{appendix:proofs}, along with the proof of \cref{thm:qot_as_registration}.
Similarly, the effective cost of \cref{eq:quad_minmax} takes the form:
\begin{equation}
\label{eq:effective_cost_decomp_blockseparable}
    c_{\Gamma,\Xi}(x,y) = - \scal{\begin{pmatrix}
        \Phi_A(x) \\ \Phi_B(x) \end{pmatrix},\begin{pmatrix}
        -\Xi \cdot \Psi_A(y) \\ \Gamma \cdot \Psi_B(y) \end{pmatrix}}.
\end{equation}


==> dual.tex <==


Reformulating matching as registration problems allows to exhibit a nested minimization structure that can be solved locally by alternate optimization over the two sets of parameters, $\Gamma$ and $\pi$.
Since the problem is convex on $\pi$, we can use any off-the-shelf convex optimization solver to update this parameter.
Yet, this kind of strategy faces an important limitation: it requires to optimize explicitly over the full coupling $\pi$.
When the regularization over $\pi$ is dualizable, we can prevent this bottleneck by adapting classical optimal transport techniques to the general matching case.
It relies on a duality result for DC functions introduced in \cite{toland1978duality}, and that provides the following equivalence:

\begin{restatable}[Toland Duality]{theorem}{toland_duality_general}
If $\Reg$ a dualizable regularizer with dual data $(\Phi, \mathcal{D}_\Reg)$ as in \cref{def:dualizable}. 
Let $\mathcal{F}^*$ and $\mathcal{G}^*$ be the convex conjugates of $\mathcal{F}$ and $\mathcal{G}$.
The matching problem
\begin{equation*}
    \min_{\pi \in \measplus{\X \times \Y}} ~~ \mathcal{F}(\pi) - \mathcal{G}(\pi) + \mathcal{R}(\pi)
\end{equation*}
is equivalent to:
\begin{equation}
\label{eq:toland_dual}
    \min_{\Gamma \in \C(\X \times \Y)}~~ \max_{\Xi \in \C(\X \times \Y)} ~~ \sup_{\phi \in \Phi} ~~ 
            \mathcal{D}_\Reg\bigl(\phi;\, \Gamma - \Xi,\, \alpha, \beta\bigr) + \mathcal{G}^*(\Gamma) - \mathcal{F}^*(\Xi).
\end{equation}
It is also equivalent to:
\begin{equation*}
\label{eq:toland_primal}
       \min_{\Gamma \in \C(\X \times \Y)}~~ \max_{\Xi \in \C(\X \times \Y)} ~~ \min_{\pi \in \measplus{\X \times \Y}} ~~ 
            \int (\Gamma - \Xi) \diff\pi + \mathcal{G}^*(\Gamma) - \mathcal{F}^*(\Xi) + \Reg(\pi). 
\end{equation*}
\end{restatable}
Therefore, up to the introduction of auxiliary variables $\Gamma$ and $\Xi$, DC matching problems can be solved by sequence of primal (\cref{eq:toland_primal}) or dual (\cref{eq:toland_dual}) OT problems, for which efficient numerical methods exist.
In the quadratic matching case, this translates as follows:

\begin{restatable}{theorem}{generalminimax}
    \label{thm:general_minmax}
The problem of \cref{eq:ugw_dc} is equivalent to:
    \begin{equation}
            \label{eq:general_minmax}
            \min_{\Gamma \in \img{B}}\;
            \max_{\Xi \in \img{A}}\;
            \sup_{\phi \in \Phi}\;
            \mathcal{D}_\Reg\bigl(\phi;\, c_{\Gamma,\Xi},\, \alpha, \beta\bigr) - \tfrac{1}{2}\norm{\Xi}^2 + \tfrac{1}{2} \norm{\Gamma}^2,
    \end{equation}
    with the effective cost
    \begin{equation*}
        c_{\Gamma,\Xi}(x,y) \;:=\; (A^*\Xi)(x,y) - (B^*\Gamma)(x,y) = \scal{\Xi, A(x,y)} - \scal{\Gamma, B(x,y)}.
    \end{equation*}
\end{restatable}
When $A$ and $B$ are separable, the effective cost can be put under the form of a simple scalar product:
\begin{equation}
\label{eq:effective_cost_decomp}
    c_{\Gamma,\Xi}(x,y) = - \scal{\begin{pmatrix}
        \Phi_A(x) \\ \Phi_B(x) \end{pmatrix},\begin{pmatrix}
        -\Xi \Psi_A(y) \\ \Gamma \Psi_B(y) \end{pmatrix}},
\end{equation}
where the parentheses indicate the direct sum (or the \emph{concatnation}) of the vectors inside it.
This new formula involves dual OT parameters $\phi$ and a new variable $\Xi$ instead of the full transport plan $\pi$.
Hence, solving the dual problem do not require to manipulate transport plans explicitly.


==> dualizable_regularizers.tex <==

In \cref{table:regularizers} and \cref{table:regularizers_dual}, we introduce the main regularizers encountered in the matching literature and their duals. 
They all follow the same structure, thoroughly studied in \cite{sejourne2022generalized}:
\begin{multline}
    \label{eq:csiszar_regs}
    \Reg(\pi) = \Div{\varphi_1}{\pi_1}{\alpha} + \Div{\varphi_2}{\pi_2}{\beta} + \varepsilon \KL(\pi \Vert \alpha \otimes \beta) \\ \text{ with } \quad \Div{\varphi}{\mu}{\nu} := \begin{cases} \int \varphi \left(\frac{\diff\mu}{\diff \nu}\right)\diff\nu & \text{ if } \mu \ll \nu, \\
    + \infty & \text{otherwise}.
    \end{cases}
\end{multline}

The function ${\rm D}_{\varphi}$ is called the Csisz\'ar divergence associated to the function $\varphi$.
It is well-defined as soon as $\varphi$ is convex and $\varphi(1) = 0$.
Regularizers like \cref{eq:csiszar_regs} are dualizable: the space of dual variables is $\Phi = \C(\X) \times \C(\Y)$, and:
\begin{equation*}
  \mathcal{D}((f,g),c,\alpha,\beta) = - \int \varphi_1^*(-f)\diff\alpha - \int  \varphi_2^*(-g)\diff\beta - \varepsilon\int(e^{(f\oplus g - c)/\varepsilon} - 1)\,\diff\alpha\otimes\beta,
\end{equation*}
where $\varphi^*_1$ and  $\varphi^*_2$ are the convex conjugates of $\varphi_1$ and $\varphi_2$.

This class of regularizers also encompasses the most classical method used in registration methods: closest point matching, or nearest neighbors.
Given a cost function $c$, it is given by:
\begin{equation*}
    \pi_{\rm CP}(x,y) = \begin{cases}
        \alpha(x) & \text{if }  y \in \arg\min_x c(x,y), \\
        0 & \text{otherwise}.
        \end{cases}
\end{equation*}
Closest point matchings are the solutions of a $\Reg\OT$ problem of the form $\min_\pi \int c\diff\pi + \Reg(\pi)$, where $\Reg$ is explicited in \cref{table:regularizers}.
This makes closest point methods entirely compatible with our framework.

\begin{table*}[h!]
  \caption{List of classical regularizers.}
  \label{table:regularizers}
\begin{tabularx}{\textwidth}{ll}
\toprule
Regularizer & $\Reg(\pi)$  \\
\midrule
Classical OT & $\iota_{\Pi(\alpha,\beta)}(\pi)$ \\
Closest Point & $\iota_{\alpha}(\pi_1)$ \\
Entropic OT & $\iota_{\Pi(\alpha,\beta)}(\pi) + \varepsilon \KL(\pi \Vert \alpha \otimes \beta)$ \\
Semi-Balanced EOT & $\iota_{\alpha}(\pi_1) + \varepsilon \KL(\pi \Vert \alpha \otimes \beta)$ \\
Unbalanced OT & $\rho_1 \KL(\pi_1, \Vert \alpha) + \rho_2 \KL(\pi_2 \Vert \beta) + \varepsilon \KL(\pi \Vert \alpha \otimes \beta)$ \\
Partial OT &  $\rho_1 \TV(\pi_1 \Vert \alpha) + \rho_2 \TV(\pi_2 \Vert \beta) + \varepsilon \KL(\pi \Vert \alpha \otimes \beta)$ \\
\bottomrule
\end{tabularx}
\end{table*}

\begin{table*}[h!]
  \caption{Dual functions of the regularizers.}
  \label{table:regularizers_dual}
\begin{tabularx}{\textwidth}{ll}
\toprule
Regularizer & $\mathcal{D}((f,g), \alpha, \beta)$ \\
\midrule
Classical OT & $ \int f\diff\alpha + \int g \diff \beta + \iota_{f \oplus g \leq c}(f,g)$ \\
Closest Point & $\int f \diff \alpha + \iota_{f(x) = \min_y c(x,y)}(f)$ \\
Entropic OT & $\int f \diff\alpha + \int g \diff \beta - \varepsilon\int(e^{(f\oplus g - c)/\varepsilon} - 1)\,\diff\alpha\otimes\beta$ \\
Semi-Balanced EOT & $\int f \diff \alpha - \varepsilon\int(e^{(f\oplus 0 - c)/\varepsilon} - 1) \diff\alpha\otimes\beta $ \\
Unbalanced OT & $\rho_1\!\int(1 - e^{-f/\rho_1})\diff\alpha + \rho_2\!\int(1 - e^{-g/\rho_2})\diff\beta
    - \varepsilon\!\int\bigl(e^{(f\oplus g - c)/\varepsilon} - 1\bigr)\diff\alpha\otimes\beta$ \\
Partial OT &  $\int \min(\rho_1, f) \diff \alpha + \int \min(\rho_2, g) \diff \beta - \varepsilon\!\int\bigl(e^{(f\oplus g - c)/\varepsilon} - 1\bigr)\diff\alpha\otimes\beta $  \\

\bottomrule
\end{tabularx}
\end{table*}

==> factorization.tex <==

\subsection{General DC Decomposition of Matching Problems}
\label{appendix:general_matching}

We now provide several existence theorems for the decomposition of matching objectives in a difference of convex functions.


\paragraph{General matching approximation by DC functions.} First, DC functions are dense in spaces of compactly-supported continuous functions.
It ensures that continuous matching objectives can be approximated by a difference of convex functions on meaningful domains for the minimization, provided that the objective grows arbitrarily at infinity:

\begin{restatable}{proposition}{densitydcfunctions}
\label{prop:density_dc_functions}
Let assume that $\Engy$ is continuous for the weak-* convergence and goes to infinity at infinity.
Then, for any precision degree $\delta > 0$, there exists a bounded convex set $V \subset \measplus{\X \times \Y}$ containing all the minima of $\Engy$ and two convex functions $\Cvxa_\delta$, $\Cvxb_\delta$ such that:
\begin{equation*}
\text{For all } \pi \in V, \quad \abs{\Engy(\pi) - \Cvxa_{\delta}(\pi) + \Cvxb_{\delta}(\pi)} < \delta,
\end{equation*}
and $ \Cvxa_{\delta}(\pi) - \Cvxb_{\delta}(\pi) = + \infty$ for $\pi \notin V$.
\end{restatable}

When $\X$ and $\Y$ are finite spaces of size $\NN$ and $\MM$, the set $\meas{\X \times \Y}$ can be identified with the Euclidean space $\R^{\NN \times \MM}$. 
If $\Engy$ is $\C^2$, \cite{hartman1959functions,hiriart1985generalized} proved that it admits an \emph{exact} DC decomposition over the whole space $\R^{\NN \times \MM}$: in this case, the DC hypothesis is always satisfied.
We refer to \cite{hiriart1985generalized} for other characterizations of DC decomposable functions.
Besides, when $\Cvxa$ and $\Cvxb$ are superlinear, their convex conjugates are continuous.
We state this result in the following lemma:

\begin{restatable}{lemma}{lemmacontinuityconjugate}
\label{lemma:continuity_conjugate}
Let assume that $\Cvxa$ is superlinear:
\begin{equation*}
    \frac{\Cvxa(\pi_n)}{\TV(\pi_n)} \longrightarrow + \infty \quad \text{ for all } (\pi_n) \in \meas{\X \times \Y} \quad \text{ such that } \quad \TV(\pi_n) \longrightarrow \infty,
\end{equation*}
with $\TV(\pi)$ denoting the total variation of $\pi$.
Then, the convex conjugate $\Cvxb^*$ is continuous on $\C(\X \times \Y)$ for the uniform norm.
\end{restatable}

Since adding the same term to $\Cvxa$ and $\Cvxb$ will always yield the same difference, we can always enforce the DC decomposition to have superlinear terms by adding the function $\pi \mapsto \TV(\pi)^2$ to both $\Cvxa$ and $\Cvxb$.
Therefore, we can always enforce the continuity of the convex conjugates $\Cvxa^*$ and $\Cvxb^*$ without any additional hypothesis.

\paragraph{Factorizability of quadratic operators.} In the finite case, the spectral theorem ensures that quadratic operators always admit a factorization like \cref{eq:loss_factorized} given by the separation of the matrix $[k(x_i,y_j,x_k,y_l)]_{(ij),(kl)}$ in positive and negative eigenspaces.
Similarly, a coordinate-wise singular value decomposition of the matrices $[A(x_i,y_j)]_{ij}$ and $[B(x_i,y_j)]_{ij}$ ensures that the quadratic operators of \cref{eq:loss_factorized} are block-separable when the inputs are finite.

This result does not hold when $\alpha$ and $\beta$ are continuous: spectral decompositions are Hilbert-related notions, whereas $\meas{\X \times \Y}$ is only a Banach space.
Yet, in entropic-regularized settings, we prove that $\Reg\QM$ optimization can be restricted to the space of couplings with squared-integrable density with respect to $\alpha \otimes \beta$:
\begin{equation*}
    \mathcal{M}^{L^2}(\alpha\otimes\beta) := \left\{ \pi \in \meas{\X \times \Y} ~~ \text{ s.t. } ~ \exists f \in L^2(\X \times \Y, \alpha\otimes\beta), \quad \pi = f \diff\alpha\otimes\beta  \right\}.
\end{equation*}
Since $L^2(\X \otimes \Y, \alpha\otimes\beta)$ is a Hilbert space, this allows us to diagonalize the kernel and prove:
\begin{restatable}{proposition}{existencediagqm}
\label{prop:existence_diag_qm}
If $\Reg$ contains an entropic term, $k$ is continuous and $\alpha,\beta$ have compact support, then there exists two linear operators $A, B : \mathcal{M}_+^{L^2}(\alpha\otimes\beta) \to L^2(\X \times \Y, \alpha\otimes \beta)$ such that:
\begin{equation*}
    \Reg\QM(\alpha, \beta) = \inf_{\pi \in \mathcal{M}_+^{L^2}(\alpha\otimes\beta)} \tfrac{1}{2} \norm{A[\pi]}^2 - \tfrac{1}{2} \norm{B[\pi]}^2 + \Reg(\pi).
\end{equation*}
with $\mathcal{M}_+^{L^2}(\alpha\otimes\beta)$ denoting the subset of positive measures of  $\mathcal{M}^{L^2}(\alpha\otimes\beta)$.
\end{restatable}
The setting is slightly different from the hypotheses of our article, but our duality results still apply and we can straightforwardly adapt our contributions to this particular case.
It evidences the naturality of quadratic operator factorization when working with entropic-regularized matching, suggesting that the reformulations we propose in \cref{section:quadratic_matching_case} are more than a numerical trick and display a fundamental property of quadratic matching problems.

\subsection{Explicit decompositions of Gromov-Wasserstein kernels}
\label{appendix:gw_decomposition}

In this section, we explain how to factorize Gromov-Wasserstein (GW) kernels of the form:
\begin{equation*}
    k(x,y,x',y') =  \bigl(c_\X(x,x') - c_\Y(y,y')\bigr)^2,
\end{equation*}
depending on the properties of the base costs $c_\X$ and $c_\Y$.
Our computations mainly rely on the following characterization lemma:
\begin{restatable}{lemma}{kernelfactorization}
    \label{lem:kernel_factorization}
    Let $k : (\X \times \Y)^2 \to \R$ be symmetric and let $A : \X \times \Y \to \Hilb_A$, $B : \X \times \Y \to \Hilb_B$. The identity
    \begin{equation*}
        \frac{1}{2} \int k\,\diff\pi\otimes\pi \;=\; \frac{1}{2} \norm{A[\pi]}^2 - \frac{1}{2} \norm{B[\pi]}^2
    \end{equation*}
    holds for all $\pi \in \meas{\X \times \Y}$ if and only if, for all $x,x'\in \X$ and $y,y' \in \Y$:
    \begin{equation*}
        k(x,y,x',y') \;=\; \scal{A(x,y), A(x',y')} - \scal{B(x,y), B(x',y')}.
    \end{equation*}
\end{restatable}

\paragraph{Inner Products and Squared Norms} When $c_\X$ and $c_\Y$ are scalar products, the kernel is a polynomial of $x$, $x'$,$y$ and $y'$, which allows us to rearrange the terms in the desired way.

\begin{proposition}
    \label{prop:scalar_decomp}
      The scalar product kernel is equivalent to:
    \begin{multline*}
        \bigl(\scal{x, x'}^2 - \scal{y, y'}^2\bigr)^2 \;=\; \scal{A(x,y), A(x',y')} - \scal{B(x,y), B(x',y')} \\
        \text{ with } \quad 
        A(x,y) =
        \begin{pmatrix}
            xx^\top                              \\
            yy^\top                              \\
        \end{pmatrix}
         \text{ and }
        B(x,y) = \sqrt{2}\, xy^\top,
    \end{multline*}
    the matrix notation denoting the direct sum of the cells (as detailed in \cref{appendix:block_separable}).
\end{proposition}

A similar decomposition can be obtained when costs are differences of scalar products:

\begin{proposition}
    \label{prop:general_decomp}
    Let $c_\X: \X \times \X \rightarrow \R$ and $c_\Y: \Y \times \Y \rightarrow \R$ such that for all $x,x' \in \X$ and $y,y' \in \Y$:
    \begin{equation*}
     c_\X(x,x') = \scal{x_+, x'_+} - \scal{x_-, x'_-} 
     \quad  \text{and} \quad 
     c_\Y(y,y') = \scal{y_+, y'_+} - \scal{y_-, y'_-}.
    \end{equation*}
    Then,
    \begin{multline*}
        \bigl(c_\X(x, x') - c_\Y(y,y')\bigr)^2 \;=\; \scal{A(x,y), A(x',y')} - \scal{B(x,y), B(x',y')} \\
        \text{ with } \quad 
    A(x, y) = \begin{pmatrix} x_+ x_+^T \\ 
     x_- x_-^T \\ 
    y_+ y_+^T  \\
    y_- y_-^T  \\
    \sqrt{2}x_- y_+^T \\
    \sqrt{2} x_+ y_-^T
    \end{pmatrix} 
    \quad \text{ and } \quad 
    B(x,y) = \begin{pmatrix} 
    \sqrt{2} x_+ x_-^T  \\
    \sqrt{2} y_+ y_-^T  \\
    \sqrt{2} x_+  y_+^T \\
    \sqrt{2} x_- y_-^T
\end{pmatrix}.
\end{multline*}
\end{proposition}    

Although these costs are never used explicitly in practice, most GW instances can be reduced to this cost structure.  
Notably, squared Euclidean norms can be rewritten as differences of scalar products:
\begin{equation*}
    \norm{x - x'}^2 =  \scal{x_+, x'_+} - \scal{x_-, x'_-}, \quad \text{ with } \quad x_+ = \tfrac{1}{\sqrt{2}} (\norm{x}^2 + 1) 
    ~ \text{ and } ~ x_- = \begin{pmatrix}
        \sqrt{2} x \\ \tfrac{1}{\sqrt{2}} (\norm{x}^2 - 1)
    \end{pmatrix}.
\end{equation*}
Therefore, a kernel factorization in the form of \cref{eq:loss_factorized} can be explicitly obtained in the classical squared norm case as well.

\begin{remark}[The balanced case]
When we restrict $\pi$ to the set $\mathcal{M}(\alpha,\beta)$ of balanced transport plans, i.e. $\pi_1 = \alpha$ and $\pi_2 = \beta$, the kernel decompositions can be further simplified.
Indeed, most terms of $a$ and $b$ only depend on either $x$ or $y$: therefore, they remain constant when the marginals of $\pi$ are fixed and hence do not play a role in the minimization.
In the balanced case, we can therefore use the following factorization:
\begin{equation*}
    \frac{1}{2} \int (\scal{x,x'} - \scal{y,y'})^2\diff\pi\otimes\pi = {\rm Cste}(\alpha,\beta) - \norm{\int xy ^T \diff\pi}^2,
\end{equation*}
and in the case of \cref{prop:general_decomp}:
\begin{equation*}
    \frac{1}{2} \int (c_\X(x,x') - c_\Y(y,y'))^2\diff\pi\otimes\pi = {\rm Cste}(\alpha,\beta) + \norm{\int \begin{pmatrix} x_-y_+^T \\ x_+y_-^T \end{pmatrix} \diff\pi}^2 - \norm{\int \begin{pmatrix} x_+y_+^T \\ x_-y_-^T \end{pmatrix} \diff\pi}^2.
\end{equation*}
Finally, for the squared norm case, the restriction of the kernel on the space $\mathcal{M}(\alpha,\beta)$ is linear in some directions of the space, allowing to write:
\begin{equation*}
    \frac{1}{2} \int (\norm{x-x'}^2 - \norm{y-y'})^2\diff\pi\otimes\pi = {\rm Cste}(\alpha,\beta) - 4 \norm{\int xy ^T \diff\pi}^2 - 2 \int \norm{x}^2 \norm{y}^2 \diff\pi,
\end{equation*}
giving the same factorization as in \cite{rioux2024entropic,zhang2024gromov}.
\end{remark}

\paragraph{Embeddable costs.} Although the previous decompositions are specific to scalar products or squared norms, they can be extended to any \emph{embeddable costs}, i.e. to costs that can be represented as a squared norm or scalar product in a certain embedding space.
There are two important categories of such costs: costs of positive and conditionally of negative type. 
We briefly introduce their theory here, refering to \cite[Appendix C]{bekka2007kazhdan} for a detailed introduction to this rich theory.

\begin{definition}[Cost of positive type]
\label{def:positive_type}
A cost $c: \X \times \X \rightarrow \R^+$ is of positive type if it is symmetric and is such that for any finite collection of points $x_1,\dots, x_n \in \X$ and coefficients $\lambda_1,\dots,\lambda_n \in \R$:
\begin{equation*}
\sum_{i=1}^n \lambda_i \lambda_j \cdot c(x_i, x_j) \geq 0.
\end{equation*}
\end{definition}

\begin{definition}[Cost conditionally of negative type]
\label{def:cnt}
A non-negative cost $c: \X \times \X \rightarrow \R^+$ is conditionally of negative type (CNT) if it is symmetric, satisfies $c(x, x) = 0$ for all $x \in \X$ and 
is such that for any finite collection of points $x_1,\dots, x_n \in \X$ and coefficients $\lambda_1,\dots,\lambda_n \in \R$:
\begin{equation*}
  \sum_{i=1}^n \lambda_i = 0 ~~\Longrightarrow~~ \sum_{i=1}^n \lambda_i \lambda_j \cdot c(x_i, x_j) \leq 0~.
\end{equation*}
\end{definition}

The following theorems show that they are indeed embeddable:

\begin{theorem}[\cite{aronszajn1950theory}]
\label{theorem:positive_embedding}
Let $c$ be a continuous symmetric function on $\X \times \X$. The cost $c$ is positive if and only if there exists a real Hilbert space $\Hilb$ and a continuous mapping $\varphi : \X \rightarrow \Hilb$ such that
for all  $x$ and $x'$ in $\X$,
\begin{equation*}
     \quad c(x, x') ~=~ \scal{\varphi(x), \varphi(x')}.
\end{equation*}
\end{theorem}

\begin{theorem}[\cite{schoenberg1938metric}]
\label{theorem:cnt_embedding}
Let $c$ be a continuous symmetric function on $\X \times \X$ satisfying $c(x,x) = 0$. The cost $c$ is CNT if and only if there exists a real Hilbert space $\Hilb$ and a continuous mapping $\varphi : \X \rightarrow \Hilb$ such that
for all  $x$ and $x'$ in $\X$,
\begin{equation*}
     \quad c(x, x') ~=~ \norm{\varphi(x) - \varphi(x')}_{\Hilb}^2.
\end{equation*}
\end{theorem}

Many important examples fall in these categories.
First, note that these categories are stable by sum and rescaling by positive coefficients.
Moreover, if two costs $c_1, c_2$ are positive, then $c_1 \cdot c_2$ is positive as well: in particular, any non-negative integer power $c^k$ of a positive cost is positive.
On the other hand, tree distances, hyperbolic geodesic distances, spherical distances and all (non-squared) Euclidean distances are CNT.
Moreover, if $c$ is CNT, then $c^p$ is CNT as well if $0 < p \leq 2$: in particular, $c(x,x') = \norm{x-x'}^p$ if CNT for any positive $p$ smaller than $2$.

\begin{theorem}
Let $c$ be a symmetric function on $\X \times \X$ with $c(x,x) = 0$.
Let $x_0 \in \X$.
The following conditions are equivalent:
\begin{enumerate}
    \item The cost $c$ is CNT,
    \item The cost $k: x,x' \in \X\times\X \mapsto c(x,x_0) + c(x_0,x') - c(x,x')$ is positive,
    \item The cost $e^{-\lambda c}: x,x' \in \X\times\X \mapsto \exp(-\lambda c(x,x'))$ is positive for every $\lambda \geq 0$.
\end{enumerate}
\end{theorem}

Although the embeddings provided by \cref{theorem:positive_embedding,theorem:cnt_embedding} are potentially infinite-dimensional, when working with finite number of points, they are restricted to a finite-dimensional subspace of the initial embedding space. 
Therefore, the embeddings can be obtained simply by diagonalizing the cost matrix defined by $c(x,x')$ in the positive type case, or the matrix defined from $c(x,x_0) + c(x_0,x') - c(x,x')$ in the CNT case.
For inputs of size $\NN$, this provides $\NN$-dimensional embeddings for these points.

\paragraph{Arbitrary costs on finite spaces.} For general cost functions, when $\X$ and $\Y$ are finite, the spectral theorem allows us to reexpress the base costs as difference of positive costs, allowing us to use the same kind of computations as in the scalar product case.
\begin{proposition}
\label{prop:diag_costs}
    Let assume that $\X$ is finite, and let $c: \X \times \X \longrightarrow \R$.
    Then, there exists two functions $\varphi_+ : \X \longrightarrow \R^{D_+}$ and $\varphi_- : \X \longrightarrow \R^{D_-}$ such that:  
    \begin{equation*}
        \text{For all } x, x' \in \X, \quad c(x,x') = \scal{\varphi_+(x), \varphi_+(x')} - \scal{\varphi_-(x), \varphi_-(x')}.
    \end{equation*}
\end{proposition}
Therefore, using \cref{prop:general_decomp} together with the diagonalization of the costs $c_\X$ and $c_\Y$, all GW losses can be put in the form of \cref{eq:loss_factorized}. 
Unlike diagonalizing the operator $k$ explicitely, diagonalizing the costs is numerically tractable and has a negligible computational cost compared to solving the GW problem, and recasting GW in the factorized form is suited for practical applications.

==> implementation.tex <==

Beyond its convergence guarantees, our algorithm offers several practical advantages worth highlighting.
Additional details on our actual implementation are given in \cref{appendix:detailed_implementation}.

\paragraph{Compatibility with generic $\Reg\OT$ backends.} Any optimal transport solver can be plugged in the $\Reg\OT$ block, allowing our $\Reg\QOT$ pipeline to directly inherit the performances of any state-of-the-art OT backend.
To ensure the highest level of compatibility, a main constraint remains to be addressed.
Indeed, most $\Reg\OT$ solvers are not compatible with generic costs functions $c$ but are rather restricted to particular cases, the most commonly supported being:
\begin{equation*}
    c(x,y) = \norm{x - y}^2 \quad \text{or} \quad c(x,y) = - \scal{x, y}.
\end{equation*}
When the operators $A$ and $B$ are separable, \cref{eq:effective_cost_decomp} shows that the effective cost $c_{\Gamma, \Xi}$ can be expressed as an inner product, ensuring compatibility with almost all existing OT backends. 
Moreover, these libraries typically provide efficient implementations of integrals of the transport plan of the form:
\begin{equation}
\label{eq:transport_integrals}
    v(x) = \int u(y) \diff\pi(x,y) \quad \text{ or } \quad   v(y) = \int u(x) \diff\pi(x,y).
\end{equation}
In the separable case, the linear operators $A[\pi]$ and $B[\pi]$ are cross-correlation operators in a lifted feature space which can be decomposed as operations like \cref{eq:transport_integrals}:
\begin{equation}
\label{eq:primal_corr}
    A[\pi] = \int \Phi_A(x)\Psi_A^{\top}(y) \diff\pi(x,y) \quad \text{ and } \quad B[\pi] = \int \Phi_B(x)\Psi_B^{\top}(y) \diff\pi(x,y).
\end{equation}
Therefore, we can implement the $\Xi$ and $\Gamma$ updates of our algorithm using standard OT operations without having to explicitly integrate over the current transport plan $\pi(\Xi, \Gamma, \Phi)$.
This allows to increase the implementation efficiency while limiting all transport-plan related operations to standard and minimal interfaces with the $\Reg\OT$ solver.
This is detailed in \cref{alg:ugw_sinkhorn}, where \texttt{Sink} represents any black-box $\Reg\OT$ solver for the cost $c(x,y) = -\scal{x, y}$, $\texttt{Sink.optimization\_step()}$ applies one update of $\phi$, and $\texttt{Sink.Corr(}A\texttt{)}$ computes the cross-correlation of $A$ for the current Sinkhorn plan.

This plug-and-play design makes the algorithm fully GPU-compatible, allows the use of linear memory OT backends, and allows to adapt the solver based on the setting (regularization type, data structure, dimensionality regime, etc.). 

\input{resources/algorithms/RQOT_separable}

\paragraph{Acceleration with multiscaling.} The optimal potentials $\Gamma$ and $\Xi$ depend on the geometry of the inputs $\alpha$ and $\beta$, rather than their precise pointwise configuration.
Replacing the inputs by coarse approximations $\alpha_c \approx \alpha$ and $\beta_c \approx \beta$ therefore yields optimal potentials $(\Gamma^*_c, \Xi^*_c)$ that remain close to the true optimum.
This motivates a natural multiscale strategy: solve the coarse problem, then initialize the fine problem using $(\Gamma^*_c, \Xi^*_c)$.
The coarse variables $\phi^*_c$ can also serve to initialize the fine-scale solver via standard OT multiscaling techniques \cite{feydy2020fast}, substantially reducing the number of iterations needed for convergence.
Similarly, since the coarse plan $\pi^*_c$ approximates $\pi^*$, a near-zero entry $\pi^*_c(x_c,y_c) \approx 0$ indicates that any fine-scale pair $(x,y)$ with $x \approx x_c$ and $y \approx y_c$ is also unlikely to be matched.
We can thus estimate sparsity masks from the coarse solution that indicates which coefficients of the final coupling are expected to be nearly zero, allowing compatible OT backends like KeOps to skip these non-relevant coefficients during computation.

\paragraph{Landmarks and minima exploration.} Since the non-convex part of the QOT problem is completely captured by the operator $B$, the local minimum reached by the algorithm is fully determined by the initial value of $\Gamma$.
The optimization landscape can therefore be explored by sampling multiple $\Gamma$ initializations.
Alternatively, when partial correspondences (landmarks) between inputs are available as prior information, they can be encoded directly in the initialization of $\Gamma$, effectively guiding the algorithm towards more meaningful local solutions.
It is finally possible to initialize the algorithm using the output of an other matching algorithm like fast rigid registration methods.
Overall, our method is sufficiently polyvalent to enable the use of the most common global minimization strategies.

==> linearizing_qot.tex <==

Scaling quadratic matching on large inputs is challenging for two main reasons.
First, quadratic matching problems are non-convex, making them hard to solve globally.
Second, the objective involves an integration over the product $\pi \otimes \pi$, which is prohibitively expensive to compute in practice and which makes even local minimization hard to perform.
These issues have been tackled in some specific cases by reformulating the optimization objective into a simpler one \citep{rioux2024entropic,zhang2024gromov,sebbouh2024structured,houry2026gromov}. 
In this section, we provide a systematic generalization of their results for arbitrary matching problems.
More specifically, we focus on matching problems where the objective is a difference of convex (DC) function:
\begin{equation}
\label{eq:dc_matching}
    \min_{\pi \in \measplus{\X \times \Y}} \mathcal{E}(\pi) \quad \text{ where } \quad \mathcal{E}(\pi) = \mathcal{F}(\pi) - \mathcal{G}(\pi).
\end{equation}

Note that any sufficiently regular matching problem can be approximated by a DC matching problem: therefore, this hypothesis is rather mild in practice.
For this class of matching problems, we prove the following reformulation:

\begin{restatable}{theorem}{thm_ccv_duality_general} \textbf{[Vérifier]}Equation~\ref{eq:dc_matching} is equivalent to:
    \begin{equation}
    \label{eq:general_matching_dualccv}
        \min_{\Gamma \in \C(\X \times \Y)} ~ \min_{\pi \in \measplus{\X \times \Y}}\; -\int \Gamma(x,y) \diff \pi(x,y) + \mathbf{R}(\pi) + \mathbf{S}(\Gamma),
    \end{equation}
    where $\mathbf{R}(\pi)= \mathcal{F}(\pi)$ and $\mathbf{S}(\Gamma) =  \mathcal{G}^*(\Gamma)$ are convex functions.
If $\X$ and $\Y$ are compact subsets of Euclidean spaces, then there exists a sequence of continuous embeddings $\Phi : \X \to l^\infty(\R)$ and $\Psi: \Y \to l^\infty(\R)$ such that equation~\ref{eq:matching} is equivalent to:
\begin{equation}
\label{eq:general_matching_registrform}
    \min_{\Gamma \in l^1(\R)} \min_{\pi \in \measplus{\X \times \Y}} - \int \scal{\Phi(x), \Gamma \cdot \Psi(y)} \diff\pi(x,y) + \mathbf{R}(\pi) + \mathbf{S}(\Gamma),\end{equation}
where $\Gamma \cdot \Psi(y) := (\Gamma_i \Psi_i(y))_{i \geq 0}$.
\end{restatable}
Although still non-convex, this reformulation entirely isolates the non-convexity inside the outer minimization over the parameter $\Gamma$, providing a cleaner framework for analyzing and exploring the optimization landscape.
It also provides a more robust formulation of the objective: unlike $\pi$, the optimal $\Gamma$ solely depends on the global geometry of the inputs $\alpha$ and $\beta$, making it intrinsically robust to empirical noise, point resampling, or permutations.
Finally, the problem is marginally convex in $\Gamma$ and in $\pi$, opening the door to rigorous alternate minimization techniques.
This structure is very similar to an other class of methods seeking correspondences between geomeric objects called \emph{registration}.
The principle of registration is to find a deformation of the target shape $\beta$ that minimizes its spatial discrepancy relative to the source shape $\alpha$.  
Given a space of transformations $\T$ and a real-valued loss function $\Loss$, standard registration problems are phrased as:
\begin{equation}
\label{eq:registration_pb}
    \min_{\Gamma \in \T} \min_{\pi \in \meas{\X \times \Y}} \frac{1}{2} \int \Loss(x, \Gamma(y)) \diff\pi(x,y) + \mathbf{R}(\pi) + \mathbf{S}(\Gamma),
\end{equation}
where $\mathbf{R}$ and $\mathbf{S}$ are regularizers.
Many popular algorithms follow this structure, such as iterative closest points \citep{besl1992method}, robust point matching \citep{gold1994new}, coherent point drift \citep{myronenko2010point}, correlation-based registration \citep{tsin2004correlation}, functional maps \citep{ovsjanikov2012functional}, Procrustes-Wasserstein \citep{grave2019unsupervised} and other methods built upon classical OT \citep{alvarez2019towards}.
These techniques rely on the same equation structure, their differences lying in the choice of the transformation space $\T$, the loss $\Loss$ and the regularizers $\mathbf{R},\mathbf{S}$.

While highlighting a conceptual similarity between two fundamental classes of problems, \cref{eq:general_matching_registrform} is numerically impractical: the embeddings $\Phi$ and $\Psi$ are generally unknown and high-dimensional, making them unsuited for real applications.
Fortunately, in most quadratic matching instances have a simpler structure that provide explicit embeddings with a smaller dimension.
Indeed, real-world QM problems generally exhibit a DC decomposition like \cref{eq:dc_matching} involving low-rank quadratic operators.
This is the case when the QM kernel function $k$ is factorizable in the following sense:
\begin{definition}[Factorizable kernel]
We say that $k$ is factorizable if its integral is decomposable as:
\begin{equation}
\label{eq:loss_factorized}
    \frac{1}{2} \int k\diff\pi \otimes \diff\pi = \frac{1}{2} \norm{A[\pi]}^2 - \frac{1}{2} \norm{B[\pi]}^2,
\end{equation}
where $A : \meas{\X \times \Y} \to \Hilb_A$ and $B : \meas{\X \times \Y} \to \Hilb_B$ are integral operators with values in Hilbert spaces $\Hilb_A$ and $\Hilb_B$.
\end{definition}
For instance, in the finite case, the spectral theorem always provide such a factorization, by separating $k$ in positive and negative eigenspaces.
Such spectral decompositions are classical in quadratic optimization; see e.g. \cite[Theorem 5]{vavasis1995complexity}.
Gromov-Wasserstein and its variants also admits an explicit factorization that we detail in the \textbf{[APPENDIX]}.
The $\Reg\QOT$ problem then becomes:

\begin{equation}
    \label{eq:ugw_dc}
     \Reg\QOT(\alpha, \beta) = \min_{\pi \in \measplus{\X \times \Y}}\; \frac{1}{2}\norm{A[\pi]}^2 - \frac{1}{2}\norm{B[\pi]}^2 + \Reg(\pi).
\end{equation}

In this setting, the general reformulation of \cref{eq:general_matching_dualccv} becomes:

\begin{restatable}{theorem}{outermin}
    \label{prop:outer_gamma}
    Equation~\ref{eq:ugw_dc} is equivalent to:
    \begin{equation}
        \label{eq:outer_gamma}
        \min_{\Gamma \in U} \min_{\pi \in \measplus{\X \times \Y}}\; -\int \scal{\Gamma, B(x,y)} \diff \pi(x,y) + \mathbf{R}(\pi) + \mathbf{S}(\Gamma),
    \end{equation}
    with $\mathbf{R}(\pi)= \tfrac{1}{2}\norm{A [\pi]}^2 + \Reg(\pi)$, $\mathbf{S}(\Gamma) = \tfrac{1}{2} \norm{\Gamma}^2$ and $U \subset \img{B}$.
\end{restatable}
To properly recover the registration-like structure of \cref{eq:general_matching_registrform}, we must make a last hypothesis on $B$: it has to be block-separable in the following sense:
\begin{definition}[Separable function]
\label{definition:separable}
A function $B : \X \times \Y \to \Hilb_B$ is separable if there exist two embedding functions $\Phi$ and $\Psi$ such that:
\begin{equation*}
    \text{For all } x \in \X \text{ and } y \in \Y, \quad B(x,y) = \Phi(x) \Psi(y)^\top.
\end{equation*}
We say that $B$ is block-separable if there is a collection of separable functions $B_1,\dots,B_\KK$ such that $\quad \norm{B[\pi]}^2 = \norm{B_1[\pi]}^2 + \dots + \norm{B_\KK[\pi]}^2$ for all $\pi \in \meas{\X \times \Y}$.
\end{definition}
Many $\Reg\QOT$ problems of interest are explicitly block-separable, including Gromov-Wasserstein and its variants.
Under this hypothesis, $\Reg\QOT$ is equivalent to the following registration problem between embedding spaces of $\Phi$ and $\Psi$:
\begin{theorem}
\label{thm:qot_as_registration}
Let assume that $B$ is block-separable.
Let $\mathbf{R}$ and $\mathbf{S}$ be as in \cref{prop:outer_gamma}.
Then, there exists embeddings $\Phi: \X \to \Hilb_\Phi$, $\Psi: \Y \to \Hilb_\Psi$ and a compact subspace $U \subset \HS(\Hilb_\Phi,\Hilb_\Psi)$ such that \eqref{eq:ugw_dc} is equivalent to:
\begin{equation}
\label{eq:matching_as_registration}
        \min_{\Gamma \in U} \min_{\pi \in \measplus{\X \times \Y}}\; - \int \scal{\Phi(x), \Gamma \Psi(y)} \diff \pi(x,y) + \mathbf{R}(\pi) + \mathbf{S}(\Gamma).
\end{equation}
\end{theorem}
In this setting, $\Reg\QOT$ is effectively equivalent to a registration problem between known features $\Phi$ and $\Psi$.
Overall, we see that although quadratic matching is generally thought as substantially harder than registration, both actually correspond to the same class of optimization problems and can be treated in a unified framework.
The main complexity of the resolution then mainly depends on the dimension of the embeddings $\Phi$ and $\Psi$.

